Effectively Leveraging CLIP for Generating Situational Summaries of Images and Videos

Situation recognition refers to the ability of an agent to identify and understand various situations or contexts based on available information and sensory inputs. It involves the cognitive process of interpreting data from the environment to determine what is happening, what factors are involved, and what actions caused those situations. This interpretation of situations is formulated as a semantic role labeling problem in computer vision-based situation recognition. Situations depicted in images and videos hold pivotal information, essential for various applications like image and video captioning, multimedia retrieval, autonomous systems and event monitoring. However, existing methods often struggle with ambiguity and lack of context in generating meaningful and accurate predictions. Leveraging multimodal models such as CLIP, we propose ClipSitu, which sidesteps the need for full fine-tuning and achieves state-of-the-art results in situation recognition and localization tasks. ClipSitu harnesses CLIP-based image, verb, and role embeddings to predict nouns fulfilling all the roles associated with a verb, providing a comprehensive understanding of depicted scenarios. Through a cross-attention Transformer, ClipSitu XTF enhances the connection between semantic role queries and visual token representations, leading to superior performance in situation recognition. We also propose a verb-wise role prediction model with near-perfect accuracy to create an end-to-end framework for producing situational summaries for out-of-domain images. We show that situational summaries empower our ClipSitu models to produce structured descriptions with reduced ambiguity compared to generic captions. Finally, we extend ClipSitu to video situation recognition to showcase its versatility and produce comparable performance to state-of-the-art methods.

==> R1_response.tex <==
\section*{Authors' response}
\thispagestyle{empty}

We thank the reviewers for their feedback. 
We are encouraged that the reviewers found our work novel, provides valuable insights and is flexible to be applied for both image and video situation recognition.
Below, we present detailed responses to the comments raised by the reviewers.
We have also modified the paper as per the suggestions of the reviewers with the \revise{highlighted changes}.


\section*{Reviewer \#1}
\Q{} In table2, the performance gains of XTF compared to TF is marginal.

\A{} We agree that the performance gains of XTF is marginal over TF. 
given the large number of nouns (11538) in imSitu, any small improvement in value and value-all is also significant. 
Also, XTF is a more intuitive model for noun prediction and localization as it queries each image patch to determine its correspondence to the role for the verb. \\


\Q{}The experiment of Instruction-tuning VLM is not very sufficient as only VILA is tested.  As shown in Table 11, the performance of semantic role labeling is amazing but value-all is low. I think instruction tuning has the potential to achieve also good performance in value-all. I hope to see more designs and better performance in this part.

\A{} Thanks for the suggestion. 
In \cref{tab:ft_vlm_imsitu}, we have now included 3 fine-tuned VLMs -- VILA \cite{Lin_2024_CVPR}, LLaVa \cite{liu2023llava} and MiniCPM-V \cite{yao2024minicpm}, for comparison with ClipSitu XTF on image situation recognition. 
The performance of all three VLMs MiniCPM-V is similar i.e. value is high but value-all is low.
We can attribute this to the fact that all the VLMs generate nouns that are semantically similar to the ground-truth nouns for each role (as shown for VILA in \cref{fig:qual_vila}) but not the exact ground-truth nouns which leads to low value-all performance.
Therefore, it is difficult to justifiably judge VLM performance on the value-all metric that is not flexible to account for semantic similarity.\\

\Q{} While the additional contributions to ClipSitu offer valuable extensions, they could benefit from more focus than the descriptions about ClipSitu. 

\A{} Thanks for the suggestion. We have moved ClipSitu for Video Situation Recognition \cref{sec:vidsitu_revised} after ClipSitu for image situation recognition.
We have also highlighted the changes made in ClipSitu to enable video situation recognition such as, Video Event Representation with X-CLIP, Sequential Noun Generation for Roles, and Event-Aware Masking for Cross-Attention Control. 

 

\section*{Reviewer \#2}
 
\Q{} The CLIP embedding seems to improve verb performance as clear from Table 3, the boost is visible only when GT verb is not available. When the GT verb is provided ground-value drops and is much lower than previous method. This raises a concern-  the performance improvement over previous methods is only because of using CLIP embeddings that improves verb prediction, the proposed XTF transformer does not add any significant value. The current text is misleading, you should mention it clearly that the improvement is due to CLIP and then additional improvements with ablation and experiments.

\A{} We would like to clarify that in case of GT and non-GT verb setting, ClipSitu uses the CLIP embedding of the verb for noun prediction and localization (grounded-value).
In Top-1 predicted verb setting, the CLIP embedding of the top-1 verb predicted using ClipSitu Verb MLP is used for noun prediction and localization.
Therefore, the improvement in both GT and non-GT verb settings is due to both CLIP embedding and XTF model. \\


\Q{} I don't see much difference in the three methods MLP, TF, and XTF. They perform similar. Seems like a lot of unnecessary design changes for merely 0.2\% improvement from TF to XTF.

\A{} We agree that the performance gains of XTF is marginal over TF. 
However, XTF is a more intuitive model for noun prediction and localization as it queries each image patch to determine its correspondence to the role for the verb. 
Furthermore, given the large number of nouns (11538) in imSitu, any small improvement in value and value-all is also significant.  \\

\Q{} What do intend to do with role prediction? As far as I understand you are predicting roles from verbs and claim that you get $\sim$100\% performance. But you don't need it as verb to role is a deterministic mapping. It would make sense if you predict roles directly from an image. This module is unnecessary.

\A{} As roles are context specific, we cannot predict them directly from the image without predicting the verb first. 
For example, the image below can be perceived as \textit{buying} or \textit{selling} and thus, the roles are dependent on the verb. 
We have included the explanation along with the example in \cref{sec:role_pred}.\\
\begin{tabular}{c}
\includegraphics[width=0.4\linewidth]
{figures/buying_53.jpg} \\
"buying" or "selling"? GT: \underline{buying}
\end{tabular}\\

\Q{} How does role prediction helps out of domain situation recognition?

\A{} Role prediction enhances out-of-domain situation recognition by providing a structured, interpretable framework for understanding new scenarios, even when they differ significantly from the training data. 
By identifying the roles associated with actions (like "driver" in a "driving" scenario or "speaker" in a "talking" scenario), a model can generalize better to unfamiliar situations by focusing on the function of entities rather than specific objects or contexts. 
This functional understanding makes it easier for the model to recognize similar role structures in out-of-domain scenarios, even if the surface details differ, allowing it to map the actions and relationships observed in new contexts back to known patterns of interaction.

Additionally, role prediction enables models to anchor their predictions in key elements of the scene (like agents, objects, and locations), making it possible to reason about an event’s dynamics without requiring specific prior examples. For instance, a role-based model that learns the concept of "agent" and "tool" in a kitchen setting could apply a similar relational understanding to a novel setting like a workshop, by identifying who is acting and with what, without needing explicit workshop examples in training. This role-driven, abstracted understanding fosters generalization and adaptability, both of which are essential for robust out-of-domain recognition.\\

\Q{} How VLMs perform well on this task given their extensive knowledge of vision and language. It performs much better than XTF as clear from the results 95 vs 47 on value. It makes sense to use VLMs for this task. Its just a matter of instruction tuning to the situation recognition format. I don't see any value in CLIP + XTF for situation recognition with limited classes as you propose. When we already have VLMs that are CLIP+LLMs and works for all the scenarios.

\A{} We agree with the reviewer that image situation recognition evaluation is limited in the number of classes and  cannot take into account extensive world knowledge of VLM in terms of vision and language. 
In future, situation recognition benchmarks should be developed with a larger number of classes that can exploit the knowledge in VLMs. 
The evaluation criteria can also be relaxed to allow semantically similar nouns predicted by the VLM as valid alternatives.
As the endeavor for creating such a dataset and annotations is beyond the scope of this paper, we compare ClipSitu on the existing imSitu dataset.
We show that a lightweight model such as XTF with CLIP embeddings can predict all nouns for a particular verb (value-all) reasonably well compared to larger VLMs in \cref{tab:ft_vlm_imsitu}.\\


\Q{} The proposed extension to videos performs poorly when compared to previous methods on Cider. To claim comparable performance is not correct.

\A{}  We are not sure what the comment refers to as ClipSituMLP + TxD performs better on all CIDEr metrics compared to other methods that do not use object bounding boxes as shown in \cref{tab:vidsitu_sota}. 
We wanted ClipSitu to predict situations directly from the video as object bounding boxes are highly dependent on object detection accuracy and ground truth bounding boxes will not be available in practice.
Among all the metrics, ClipSitu results are lower on Lea suggesting that ClipSitu sometimes misidentify key roles with incorrect nouns, resulting in incomplete or incorrect scene interpretations. 
Lea weights each entity by its "importance" and "resolution score," a low score might suggest that ClipSitu commits ambiguous role assignments such as confusing "driver" with "passenger" weakening the accuracy and coherence of the scene interpretation.
This discussion is included in \cref{sec:vidsitu_sota}. \\


\Q{} Effectively the paper is about CLIP + Transformer. I don't see any novelty and the claims are a bit misleading. Moreover in the times of VLMs, the contribution seems not very relevant to today's state-of-the art.

\A{} Our ClipSitu models for image and video situation recognition offer a structured approach to addressing the unique challenges in this domain that differ from standard vision-language models (VLMs). 
While ClipSitu builds on the strengths of CLIP and Transformer architectures, it is specifically designed to achieve explicit and interpretable role-noun generation—a targeted improvement that serves situation recognition tasks in a way that generic fine-tuning alone often cannot match. 
This approach enables ClipSitu to deliver structured outputs that maintain contextual integrity and temporal coherence across both images and segmented video events, making it especially well-suited for complex, role-based recognition tasks as required by benchmarks like VidSitu. 
We believe this structured setup adds interpretability and precision to the model’s outputs, supporting the nuanced requirements of situation recognition more directly than traditional VLMs focused on broader tasks.\\



\section*{Reviewer \#4}
 
\Q{} The methods selected in the Table 3 of the experiment are not described. Also could be compared with some newest approaches?

\A{} We have described the methods selected for comparison in  \cref{tab:sotatable} (earlier Table 3) in \cref{sec:imsitu_sota}. The latest reported approach in literature on imSitu is CoFormer \cite{cho2022collaborative} which we have already compared with in the table. In \cref{tab:ft_vlm_imsitu}, we have also compared ClipSituXTF with 3 state-of-the-art VLMs.\\

\Q{} This paper compares with VLM, but only with VILA, which is a little monotonous. Even if its performance is optimal, it can also consider introducing LLaVA or even Video-LLMs for comparison, so that the experimental analysis will be more comprehensive.

\A{} Thanks for the suggestion. 
For image situation recognition, in \cref{tab:ft_vlm_imsitu} we have included more VLMs such as LLaVA \cite{liu2023llava} and MiniCPM-V \cite{yao2024minicpm} for comparison and the relevant discussion is in \cref{sec:tuned_vlm_imsitu}.
For video situation recognition, in \cref{tab:ft_vila_vidsitu}, we have included 3 new video LLMs such as LLaVA-Video \cite{zhang2024video}, Qwen2-VL \cite{wang2024qwen2} and MiniCPM-V \cite{yao2024minicpm} for comparison and we have discussed the results in \cref{sec:tuned_vlm_vidsitu}.
\\

\Q{} The approach part is almost consistent with the WACV 2024 paper, which seems to be not innovative in the approach. Could you consider making appropriate adjustments to the approach part based on the comparison between ClipSitu and the last paragraph of Introduction 1, such as highlighting videos or other differences from ClipSitu?

\A{} Thanks for the suggestion. 
We have moved ClipSitu for Video Situation Recognition \cref{sec:vidsitu_revised} after ClipSitu for image situation recognition.
We have elaborated the model details such as event-aware masking and loss functions.
We have also highlighted the changes made in ClipSitu to enable video situation recognition such as, Video Event Representation with X-CLIP, Sequential Noun Generation for Roles, and Event-Aware Masking for Cross-Attention Control.

